Balancing Scalability and Uniformity in SAT Witness Generator

Constrained-random simulation is the predominant approach used in the industry for functional verification of complex digital designs. The effectiveness of this approach depends on two key factors: the quality of constraints used to generate test vectors, and the randomness of solutions generated from a given set of constraints. In this paper, we focus on the second problem, and present an algorithm that significantly improves the state-of-the-art of (almost-)uniform generation of solutions of large Boolean constraints. Our algorithm provides strong theoretical guarantees on the uniformity of generated solutions and scales to problems involving hundreds of thousands of variables.

==> Analysis.tex <==
\section{Analysis}\label{sec:analysis}
In this section, we first prove the 3-wise independence of $H_{ind}(n,m,3)$ and then derive the 
lower and upper bounds on probability of generation of witnesses. Finally, we derive lower bounds 
on success probability of {\UniGen}. For lack of space, we defer the proofs of lemmas and theorems 
to Appendix. 

\begin{theorem}
$H_{ind}^{\I}(n,m,3)$ is 3-wise independent.
\end{theorem}
The following result, a slight variation of Theorem~5 
in~\cite{Schmidt}, about Chernoff-Hoeffding bounds plays an important
role in our analysis. 
\begin{theorem}\label{theorem:chernoff-hoeffding}
Let $\Gamma$ be the sum of $r$-wise independent random variables, each
of which is confined to the interval $[0, 1]$, and suppose
$\expect[\Gamma] = \mu$.  For $0 < \beta \le 1$, if $2 \le r \le \left\lfloor
\beta^{2}\mu e^{-1/2} \right\rfloor \leq 4$ , then $\prob\left[\,|\Gamma - \mu| \ge
  \beta\mu\,\right] \le e^{-r/2}$.
\end{theorem}


Let $R_F$ denote the set of witnesses of the input formula $F$. We assume $\log (|R_F|-1) - \log \mathrm{pivot}$ is an integer and denote by $m$. By the design of the algorithm, $\mathrm{pivot} \ge 17$ and if the algorithm does not return from line $6$, then $|R_F| \ge 18$. The following lemma shows that $q$ is a good estimator of $m$. 
\begin{lemma}\label{lm:mval}
$\prob [ q-3 \le m \le q] \ge 0.8$
\end{lemma}
For uniformity analysis, probabilistic analysis of the conditional check in line 16 is important. We define $w_{i,y,\alpha}$ as $\prob\left[\frac{\mathrm{pivot}}
  {1+\kappa}\right.$ $\left. \le |R_{F,h,\alpha}| \leq 1+(1+\kappa) \right.$ $\left. pivot \mbox{ and } 
  h(y) = \alpha : \right.$ $\left. h \xleftarrow{R} H_{xor}(|X|, i,
3)\right]$.

The following lemma provides lower bound on the probability of generation of a witness. The construction of the proof also provides lower bound on $w_{m,y,\alpha}$.
\begin{lemma} \label{lm:lowerBound}
For every witness $y$ of $F$, $\prob[\textrm{y is output}] \ge \frac{0.8 (1-e^{-1})}{(1.06+\kappa)(|R_F|-1)} $
\end{lemma}
 Using 3-wise independence of $H_{xor}(|X|,m,3)$, we prove the following upper bound on $w_{m,y,\alpha}$.

\begin{lemma} \label{lm:iterProof}
For $i < m$,  $w_{i,y,\alpha} \leq \frac{1}{|R_F|-1}\frac{1}
  {\left(1-\frac{1+\kappa}{2^{m-i}}\right)^2}$.
\end{lemma}
The following theorem uses Lemma ~\ref{lm:iterProof} and provides the corresponding upper bound on $\prob[\textrm{y is output}]$.
\begin{lemma}\label{lm:upperBound}
For every witness $y$ of $F$, $\prob[\textrm{y is output}] \le \frac{1+\kappa}{|R_F|-1} (2.23+ \frac{0.48}{(1-\kappa)^2})$
\end{lemma}

Combining Lemma ~\ref{lm:lowerBound} and ~\ref{lm:upperBound}, the following theorem is obtained.
\begin{theorem} \label{theorem:unigen}
For every witness $y$ of $F$ and $t > 2.7$,\\ 
 \[ \frac{1}{t}\frac{1}{|R_F|-1} \le \prob [\textrm{y is output}] \le t \frac{1}{|R_F|-1}\].
\end{theorem}


Using $3-$ wise indepndence of $H_{ind}(n,m,3)$ and Theorem ~\ref{theorem:chernoff-hoeffding}, we prove the following lower bound on success probability.


\begin{theorem}
Algorithm {\UniGen} succeeds (i.e. does not return $\bot$) with probability at least $0.62$.
\end{theorem}

\subsection*{Choice of parameter t}
One might be tempted to use smaller values of parameter $t$ to obtain better guarantees 
of uniformity as shown in Theorem ~\ref{theorem:unigen}, however there are tradeoffs 
involved. A $t$ decreases, $k$ increases and since $pviot$ is inversely proportional to 
$k$, therefore $pivot$ increases. Increased $pivot$ implies that {\BoundedSAT} has to find more 
witnesses, and therefore each invokation of {\BoundedSAT} is likely to take more time.

==> Results.tex <==
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


\begin{table*}[H]
\caption{Runtime performance comparison of {\UniGen} and {\UniWit}}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{3}{|c|}{}& \multicolumn{3}{|c|}{\UniGen} &
\multicolumn{3}{|c|}{\UniWit} \\
\hline 
Benchmark & \#Variables & Clauses &  \shortstack{Succ\\Prob} & \shortstack{Avg\\Run Time (s)}
&\shortstack{Avg\\XOR len}  & \shortstack{Avg\\Run Time (s)} & \shortstack{Avg\\XOR len} &  \shortstack{Succ\\Prob} \\
\hline


s1196a\_15\_7&777&2165&0.97&8.98&16&136.54&389\\\hline
s1196a\_3\_2&690&1805&1.0&7.12&16&501.98&343\\\hline
s1196a\_7\_4&708&1881&1.0&6.9&16&1049.02&353\\\hline
s1238a\_15\_7&773&2210&1.0&7.94&16&285.38&385\\\hline
s1238a\_3\_2&686&1850&0.99&10.85&16&1164.08&343\\\hline
s1238a\_7\_4&704&1926&1.0&7.26&16&1270.93&350\\\hline
s1488\_3\_2&854&2423&0.99&0.1&7&1.12&426\\\hline
s1488\_7\_4&872&2499&0.99&0.11&7&1.68&436\\\hline
s298\_15\_7&292&870&0.98&0.06&9&0.8&145\\\hline
s298\_7\_4&223&586&0.99&0.05&9&0.64&111\\\hline
s444\_3\_2&290&712&0.99&0.58&12&5.82&144\\\hline
s526\_15\_7&452&1303&0.99&1.68&12&23.11&225\\\hline
s526\_3\_2&365&943&0.98&0.68&12&54.91&181\\\hline
s526\_7\_4&383&1019&1.0&1.44&12&16.68&192\\\hline
s526a\_15\_7&453&1304&0.99&1.72&12&21.11&226\\\hline
s526a\_3\_2&366&944&1.0&0.97&12&82.11&183\\\hline
s526a\_7\_4&384&1020&0.99&1.5&12&17.26&192\\\hline
s820a\_15\_7&685&1987&1.0&0.18&12&5.36&341\\\hline
s820a\_3\_2&598&1627&1.0&0.08&12&1.13&297\\\hline
s820a\_7\_4&616&1703&0.99&0.15&12&2.95&307\\\hline
s832a\_15\_7&693&2017&0.99&0.74&12&21.77&345\\\hline
s832a\_3\_2&606&1657&0.99&0.1&12&1.56&304\\\hline
s832a\_7\_4&624&1733&0.99&0.2&12&4.48&311\\\hline
s953a\_3\_2&515&1297&0.99&12.48&23&22529.2&258\\\hline
LLReverse\_8\_25&63797&257657&1.0&33.92&13&2984.34&31896\\\hline
scenarios\_tree\_delete.sb.pl.sk\_3\_30&5758&22105&1.0&0.11&15&11.07&2878\\\hline
scenarios\_treemax.sb.pl.sk\_7\_19&24859&103762&1.0&0.52&10&51.94&12429\\\hline
sort.sk\_8\_52&12125&49611&0.99&79.44&26&--&6070\\\hline

SK\_51&3708&14594&1.0&12.18&19&9.72&1853\\\hline
LLReverse&63797&257657&1.0&33.75&13&3691.18&31893\\\hline
ProcessBean\_8\_64&4768&14458&0.98&123.52&32&--&2388\\\hline
ProjectService3\_12\_55&3175&11019&1.0&71.74&28&--&1591\\\hline
enqueueSeqSK\_10\_42&16466&58515&1.0&32.39&21&--&8239\\\hline
karatsuba\_7\_41&19594&82417&1.0&85.64&21&--&9771\\\hline
tutorial3.sk\_4\_31&486193&2598178&0.98&782.85&16&--&--\\\hline

\hline 
\end{tabular} 
\end{center}
\end{table*}



%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

































